Novel fluctuations at constrained interfaces

In this study we try to answer the qustion : What happens when explicit constraints are introduced such that the low energy, long wavelength modes of a system are unavailable ? This question has assumed some importance in recent years due to the advent of nano technology and the growing use of nanometer scale devices and structures. In a small system, the size limits the scale of the fluctuations and makes it imperative for us to understand how the response of the system is altered in such a situation. In this thesis, this question is answered for the special case of interfacial fluctuations in two dimensions (2d). The energy of an interface between two phases in equilibrium is invariant with respect to translations perpendicular to the plane (or line in 2d) of the interface. We study the consequence of breaking this symmetry explicity using an external field gradient. One expects that since low energy excitations are suppressed, the interface would be flat and inert at all times. We show that surprisingly there are novel fluctuations and phenomena associated with such constrained interfaces which have static as well as dynamic consequences. The Ising interface on a square lattice is shown to undergo a multitude of structural transitions as a function of velocity and the orientation. Liquid solid interfaces show coherent addition and removal of atomic layers providing novel mechanisms of stress relaxation in a nanosized single crystal without defects. We study momentum and energy transfer across the liquid solid interface in the presence of this ``layering'' transition.

==> Texfiles/dec.tex <==
{\pagestyle{empty}
\noindent
\begin {center}
 {\Large {\bf STUDY OF SCALE-FREE
 CORRELATED \\CLUSTERS IN THE
 NON-EQUILIBRIUM AND \\EQUILIBRIUM CRITICAL PHENOMENA \\ }}
\end {center}
\vskip 6.0 cm
\begin {center}
\large{\bf
THESIS  SUBMITTED FOR THE DEGREE OF \\
DOCTOR OF PHILOSOPHY (SCIENCE) \\ OF THE
UNIVERSITY OF JADAVPUR} \\
\vfill
\Large{\bf RUMANI KARMAKAR} \\
\large{SATYENDRA NATH BOSE NATIONAL CENTRE FOR BASIC SCIENCES \\
BLOCK-JD, SECTOR-III, SALT LAKE \\
KOLKATA - 700098, INDIA \\
\vskip 0.5 cm
{\bf MARCH, 2005}} \\

\end {center}
\eject
\vfill
\eject

}


%\eject

{\pagenumbering{roman}

\begin{center}
\vspace*{4cm}
{\Large \bf CERTIFICATE FROM THE SUPERVISOR}
\vspace{2.0cm}
\end{center}
%\noindent

This is to certify that the thesis entitled 
``{\bf Study of scale-free correlated clusters in the non-equilibrium and equilibrium 
critical phenomena}'' submitted by {\bf Smt. Rumani Karmakar}, who got her name
registered on {\bf July 4,2002} for the award of {\bf Ph.D.(Science) degree} of {\bf Jadavpur University},
is absolutely based upon her own work under the supervision of 
{\bf Dr. Subhrangshu Sekhar Manna} and that neither this thesis nor any part of it
has been submitted for any degree / diploma or any other academic award anywhere before.

\vskip 3.5 cm
\leftline {Date:}
\rightline {\bf Subhrangshu Sekhar Manna}
\rightline {Associate Professor}
\rightline {Satyendra Nath Bose National Centre for Basic Sciences}
\rightline {Block-JD, Sector-III, Salt Lake, Kolkata - 700098}
\vfill
\eject
%}

{\Large {\bf Acknowledgements}}
\vspace{0.6cm}

 This is my pleasure to introduce this thesis which I believe is the 
outcome of my research work during which period I have been accompanied and 
supported by a number of individuals. With pleasure I take this opportunity 
 to acknowledge my gratitude to all of them.

 First of all I am grateful to my supervisor Dr. Subhrangshu Sekhar Manna
 for all the constant encouragement, support and expert guidance he has 
provided me throughout my tenure here at the S. N. Bose National Centre for 
Basic Sciences, without which this work would not have materialized at all.  
 I thank him for being patient with me. I feel priviledged to have learnt a 
lot from his expertise and dedication to physics.

 There are so many others who needs my appreciation and I just hope  
 to remember all of them!! It was my good fortune to have some terribly
nice seniors and I learnt lots from them. I would like to thank specially 
 Aninda Jiban Bhattacharya and Atisdipankar Chakrabarti   
 for their assistance during my research period. Needless to 
say, I am amply benefitted by my colleagues  particularly Sumana, Swarnali,
 Gautam da and Durga with whom I had discussions on several topics.  
 It is my pleasure to thank all my friends at my host institution for their 
 help in many direct and indirect ways. Special mention are due to Dipankar, 
Sudeshna, Aftab, Kunal, Venkat, whose company I really enjoyed. 

 I would also like to thank my SINP friends Anirban Chakraborti, 
Arnab Chatterjee, Sutarshi Pradhan and Sucheta Adhikari who have always been so helpful. 
 I am greatly benefitted from discussions in our network group at Science 
College.
 
 I would like to extent my warmest thanks to Dr. Tapati Dutta, lecturer in 
Physics, St. Xavier's College, Kolkata for 
her collaboration in significant portion of my research work. It was a great 
pleasure working with her. Her suggestions and constant encouragement were of 
the utmost value.
 
 I thank Professor Sushanta Dattagupta, Director, S. N. Bose National
 Centre for Basic Sciences, Kolkata for the support provided by him during my 
 research work at this centre. I am grateful to Professor 
Abhijit Mookerjee, Dean of Academic Affairs of the S. N. Bose Centre, for his 
  active co-operation. I wish to acknowledge and 
express my heartfelt thanks to all the academic and non-academic staff  
members of this centre for their assistance. 

 A very special mention is deserved for Professor Monoranjan Saha, the Khaira
 Professor of physics, Calcutta University, who have been 
my mentor from my very childhood. His constant affection and encouragement 
has aroused interest in physics in me. I really feel priviledged to have 
such an eminent professor beside me.
 
 My acknowledgement is incomplete without mentioning the constant support 
and encouragement from  my parents, brothers and sisters. Last, but not the 
least, I am very much indebted to my husband, whose patience, understanding 
and encouragement helped me to fulfill my dreams. 
\vskip 1.0 cm

\rightline {\bf Rumani Karmakar}
\rightline {Satyendra Nath Bose National Centre for Basic Sciences}
\rightline {Block-JD, Sector-III, Salt Lake, Kolkata - 700098}
\vfill
\eject

{\Large {\centerline {\bf List of Publications}}}

\vskip 1.0 cm

{
\hskip -1.0 cm
\begin {itemize}
\item [1.] {\bf Precise Toppling Balance, Quenched Disorder, and Universality for Sandpiles}\\
                 R. Karmakar, S. S. Manna, and A. L. Stella \\ Phys. Rev. Lett. {\bf 94}, 088002 (2005).
\item [2.] {\bf Sandpile model on a quenched substrate generated by kinetic self-avoiding trails}\\
                 R. Karmakar and S. S. Manna \\
 Phys. Rev. E {\bf 71}, 015101 (2005).
\item [3.] {\bf Sandpile model on an optimized scale-free network on Euclidean space}\\
                 R. Karmakar and S. S. Manna\\
 J. Phys. A: Math. Gen. {\bf 38}, L87-L93 (2005).
\item [4.] {\bf Particle-hole symmetry in a sandpile model}\\
                 R. Karmakar and S. S. Manna\\
 J. Stat. Mech., L01002 (2005). 
\item [5.] {\bf Directed fixed energy sandpile model}\\
                 R. Karmakar and S. S. Manna\\
 Phys. Rev. E {\bf 69}, 067107 (2004).
\item [6.] {\bf A Percolation Model of Diagenesis }\\
                 S. S. Manna, T. Dutta, R. Karmakar and S. Tarafdar\\
 Int. J. Mod. Phys. C {\bf 13}, 319 (2002).
\item [7.] {\bf A geometrical model of diagenesis using percolation theory}\\
                 R. Karmakar, S. S. Manna and T. Dutta\\
 Physica A, {\bf 318}, 113 (2003).
\end {itemize}
}

\vfill
\eject



==> ltex <==
latex $1.tex
bibtex $1.tex
latex $1.tex
latex $1.tex
dvips $1.dvi -o $1.ps
dvipdf $1.dvi
\rm *.dvi *.aux *.log

